Fusion Dynamical Systems with Machine Learning in Imitation Learning: A Comprehensive Overview

Imitation Learning (IL), also referred to as Learning from Demonstration (LfD), holds significant promise for capturing expert motor skills through efficient imitation, facilitating adept navigation of complex scenarios. A persistent challenge in IL lies in extending generalization from historical demonstrations, enabling the acquisition of new skills without re-teaching. Dynamical system-based IL (DSIL) emerges as a significant subset of IL methodologies, offering the ability to learn trajectories via movement primitives and policy learning based on experiential abstraction. This paper emphasizes the fusion of theoretical paradigms, integrating control theory principles inherent in dynamical systems into IL. This integration notably enhances robustness, adaptability, and convergence in the face of novel scenarios. This survey aims to present a comprehensive overview of DSIL methods, spanning from classical approaches to recent advanced approaches. We categorize DSIL into autonomous dynamical systems and non-autonomous dynamical systems, surveying traditional IL methods with low-dimensional input and advanced deep IL methods with high-dimensional input. Additionally, we present and analyze three main stability methods for IL: Lyapunov stability, contraction theory, and diffeomorphism mapping. Our exploration also extends to popular policy improvement methods for DSIL, encompassing reinforcement learning, deep reinforcement learning, and evolutionary strategies.

==> macrosNew.tex <==
\usepackage{enumitem}
%\usepackage{lineno}
%\linenumbers

\usepackage[ruled,lined]{algorithm2e}
%\usepackage[ruled,linesnumbered]{algorithm2e}
\makeatletter
\newcommand{\removelatexerror}{\let\@latex@error\@gobble}
\makeatother

%\usepackage[table]{xcolor}
%\usepackage{graphics}
\definecolor{Light0}{cmyk}{0,0.03, 0.03, 0.0}
\definecolor{Light1}{cmyk}{0,0.05, 0.0, 0.05}
\definecolor{Light2}{cmyk}{0,0.05, 0.0, 0.0}
\definecolor{Light3}{cmyk}{0,0.05, 0.05, 0.05}

%\newcommand{\bm}[1]{\boldsymbol{\mathbf{#1}}}
\def\LtwoNorm{$\ell^2$norm}

\usepackage{tabularx}
\makeatletter
\newcommand{\multiline}[1]{%
	\begin{tabularx}{\dimexpr\linewidth-\ALG@thistlm}[t]{@{}X@{}}
		#1
	\end{tabularx}
}
\def\algbackskip{\hskip-\ALG@thistlm}
\makeatother

\newcommand{\TODO}[1]{\todo[inline,caption={},color=blue!30]{TODO: #1}}
\providecommand{\change }[1]{{\color{black}#1}}

\newcommand{\ToBeDeleted}[1]{\todo[inline,caption={},color=yellow!30]{\textbf{ToBeDeleted:} #1}}
\newcommand{\trsp}{{^{\top}}}

\providecommand{\matt }[1]{{\color{red}#1}}
\providecommand{\fa}[1]{{\color{blue}#1}}
\providecommand{\atY}[1]{\textcolor{violet}{@Yingbai:~}\textcolor{gray}{#1}}
\providecommand{\atF}[1]{\textcolor{violet}{@Fares:~}\textcolor{yellow}{#1}}

%% new cross-reference commands
%\newcommand{\figref}[1]{Fig.~\hyperref[#1]{\ref*{#1}}}
%\newcommand{\figsref}[1]{Figures~\hyperref[#1]{\ref*{#1}}}
%\newcommand{\Figref}[1]{Figure~\hyperref[#1]{\ref*{#1}}}
%\newcommand{\Figsref}[2]{Figures~\ref{#1}--\ref{#2}}
%\newcommand{\tabref}[1]{Tab.~\hyperref[#1]{\ref*{#1}}}
%\newcommand{\secref}[1]{Section~\hyperref[#1]{\ref*{#1}}}
%\newcommand{\algoref}[1]{Algorithm~\hyperref[#1]{\ref*{#1}}}
%\newcommand{\subfigref}[1]{(\subref{#1})}

%% Define format of some common idioms
\newcommand{\wrt} {\textit{w.r.t.}~} %
\newcommand{\eg} {{e.g.,}~} %
\newcommand{\ie} {{i.e.,}~} %
\newcommand{\etc}{\textit{etc}} %
\newcommand{\etal}{~\MakeLowercase{\textit{et al.\ }}}


\newcommand{\python}{\texttt{Python}}
\newcommand{\pytorch}{\texttt{PyTorch}}
\newcommand{\cpp}{\texttt{C++}}
\newcommand{\simulink}{\texttt{Matlab Simulink}}
\newcommand{\matlab}{\texttt{Matlab}}
\newcommand{\panda}{Franka Emika Panda}

\newcommand*\dashline{\rotatebox[origin=c]{90}{\,-\,-}}


